Exploring Explainability: A Definition, a Model, and a Knowledge Catalogue

The growing complexity of software systems and the influence of software-supported decisions in our society awoke the need for software that is transparent, accountable, and trustworthy. Explainability has been identified as a means to achieve these qualities. It is recognized as an emerging non-functional requirement (NFR) that has a significant impact on system quality. However, in order to incorporate this NFR into systems, we need to understand what explainability means from a software engineering perspective and how it impacts other quality aspects in a system. This allows for an early analysis of the benefits and possible design issues that arise from interrelationships between different quality aspects. Nevertheless, explainability is currently under-researched in the domain of requirements engineering and there is a lack of conceptual models and knowledge catalogues that support the requirements engineering process and system design. In this work, we bridge this gap by proposing a definition, a model, and a catalogue for explainability. They illustrate how explainability interacts with other quality aspects and how it may impact various quality dimensions of a system. To this end, we conducted an interdisciplinary Systematic Literature Review and validated our findings with experts in workshops.

==> content/07discussion.tex <==
\section{Discussion}
\label{sec:Discussion}
Artificial systems increasingly proliferate into all aspects of human life. Where formerly humans were decision-makers, now systems take over their jobs. With this omnipresence, aspects of ethics and safety are rapidly gaining priority. For this reason, we have to ensure that systems are well-designed. Explainability is a new NFR that echoes the demand for more human oversight of systems \cite{Thiebes2020},~\cite{EUHLEGOAI} and can bring positive consequences across all system dimensions: from users' needs to domain aspects and project constraints. It is not only important that explainability is included as a system quality, but that it is well designed and operationalized so that it has a positive impact on the system. Poor design may result in negative effects on important aspects in the system. For instance, if not properly designed, explainability can negatively affect the relationship with the user (e.g., user experience issues), interfere on important quality aspects for a corporation (e.g., damaging the brand image and the customer loyalty) and bring disadvantages for the project or the system (e.g., increasing development costs or hindering system performance).

For this reason, we should be concerned with understanding explainability as a whole: its meaning, its effects, its taxonomy. In holding this knowledge, it is possible to think of design, strategies and implementation level solutions that result in positive effects not only for the different system dimensions but also for the stakeholders involved. The model and the catalogue presented in this paper can help to recognize trade-offs as well as synergies between explainability and other quality aspects. As a result, software engineers may prevent conflicts between quality aspects and choose the best strategies for achieving the desired quality outcomes.

During our literature review, we have observed a growing need to keep explainability in mind while designing a system. We identified more than 200 works that described an influence of explainability on other quality aspects. Our literature review illustrates that there is much to do in the field of NFRs. As we have already clarified, we did not only distill traditional NFRs from our review, but widened our focus to quality aspects in general. As systems are progressing towards ever-new application fields, we believe that there may be other emerging NFRs besides explainability. Indeed, aspects such as human-machine cooperation and mental model accuracy show that there are specific needs with regard to systems when they are used to support humans. Among others, ethics, fairness, and legal compliance are all quality aspects that are gaining importance and should be better researched.

Research in RE can profit from insights of other disciplines when it comes to this regard. The fields of Philosophy, Law, and Psychology, for example, have long researched such aspects (concerning explanations, see \cite{Hempel1965} for an early source and \cite{Miller2019} for an overview). Requirement engineers might profit from insights from these disciplines. At the same time, they can guide discussions about how to include such values in systems and how to adapt development processes. This knowledge, scattered across different areas, must be made available and integrated into the day-to-day development of systems. Models and catalogues such as the ones presented in this paper can synthesize this knowledge.

Nevertheless, explainability also exhibited an impact on nearly all traditional NFRs that can be found in the ISO 25010~\cite{ISO25010}: performance efficiency, usability, reliability, security, maintanability, and portability. As such, explainability occupies a prominent role in the NFR landscape. With this work, we expect to have given a valuable input with regard to this new requirement.

==> content/07newdiscussion.tex <==
\section{Discussion}
\label{sec:Discussion}


%TODO: 1. Other disciplines
%2. Too much focus on explainability for AI, but no process

%With the omnipresence of artificial systems, aspects of ethics and safety are rapidly gaining priority.
Explainability is a new NFR that echoes the demand for more human oversight of systems \cite{Thiebes2020}. It can bring either positive or negative consequences across all quality dimensions: from users' needs to project constraints. Explainability's impact on so many important dimensions may be related to the fact that explainability can be viewed as an aspect of communication between systems and humans. Communication in human relationships can either strengthen relationships or harm them, depending on how it occurs in practice -- how we translate abstract thoughts and feelings into words. We may apply the same principle to explainability, if we consider that receiving explanations is a form of communication from a system towards its users. This fact makes explainability a valuable requirement that, as our findings show, can contribute to the achievement of several fundamental values in modern systems such as ethics, fairness, and trust. %In fact, there is empirical evidence that conversational agents can  induce  social-emotional  effects  similar  to  those  in  human-to-human  interactions [REF].

%During our literature review, we identified more than 200 works that described an influence of explainability on other quality aspects.

%This emphasises the importance of explainability in the NFR landscape. Therefore, it is not only important that explainability is included as a system quality, but that it is carefully operationalized. Bad design decisions towards explainability can negatively affect the relationship with the user (e.g., user experience issues), interfere on important quality aspects for a corporation (e.g., damaging the brand image and the customer loyalty), and bring disadvantages for the project or the system (e.g., increasing development costs or hindering system performance).

The importance of explainability in the NFR landscape emphasizes the need for greater awareness of this topic for modern systems, as well as greater understanding of its meaning. Our working definition for requirements engineers and software professionals brings up some aspects that should be explored and translated into requirements and the appropriate functionality to fulfill them. Defining the component factors of explainable systems facilitates the software engineering process, supporting the elicitation and specification of requirements, as well as the verification and validation of the corresponding explainability requirements. Bad design decisions towards explainability can negatively affect the relationship with the user (e.g., user experience issues), interfere on important quality aspects for a corporation (e.g., damaging the brand image and the customer loyalty), and bring disadvantages for the project or the system (e.g., increasing development costs or hindering system performance).  %methods and tools to assist software professionals in developing explainable systems.



Our literature review illustrates that there is much to do in the field of NFRs. We did not only distill traditional NFRs from our review, but widened our focus to quality aspects in general. As systems are progressing towards ever-new application fields, we believe that there may be other emerging NFRs besides explainability. Indeed, aspects such as human-machine cooperation and mental model accuracy show that there are specific needs with regard to systems when they are used to support humans. Among others, ethics, fairness, and legal compliance are all quality aspects that are gaining importance and should be better researched.

%During requirements specification it is necessary to define the appropriate corresponding functional requirements aligned with stakeholders' needs. In this phase, it may be necessary to count on knowledge from other disciplines. Studying the interaction between users and systems is already part of research areas such as information retrieval, usability and HCI. Recently, the research area of human-machine communication (HMC) has gained more significance, focusing on the communication and interaction between people and technology, as well as the implications for individuals and society \cite{Guzman2020}. 

%Research in RE can profit from insights of other disciplines when it comes to this regard.
When it comes to this, requirements engineers may benefit from the insights of other disciplines. The fields of Philosophy, Law, and Psychology, for example, have long researched such aspects (concerning explanations, see \cite{Hempel1965} for an early source and \cite{Miller2019} for an overview). At the same time, they can guide discussions about how to include such values in systems and how to adapt development processes. This knowledge, scattered across different areas, must be made available and integrated into the day-to-day development of systems. Models and catalogues such as the ones presented in this paper can synthesize this knowledge.

Nevertheless, explainability also exhibited an impact on nearly all traditional NFRs that can be found in the ISO 25010~\cite{ISO25010}: performance efficiency, usability, reliability, security, maintanability, and portability. As such, explainability occupies a prominent role in the NFR landscape. With this work, we expect to have given a valuable input with regard to this new requirement.


%Interactions  with  AI-enabled  devices and programs are dynamic rather than static, contingent upon the messages being exchanged within a particular moment and context or upon the data being fed into the program. Some AI technologies also are responsive to individual users, “learning” about their  human  communication  partner  and  adjusting  interactions  accordingly.  Some  


%ocuses on the theory and practice of communication with and about digital interlocutors, which may take the form of artificial conversation entities, artificially intelligent software, embodied machine communicators (robots), and technologically-augmented persons (cyborgs), as well as on communication in the context of machine spaces (virtual and augmented realities) and human-machine configurations. Additionally, the journal will publish contributions that shed light on the relationship between human and machine, as constructed through discourse and interaction. 

%testing human responses to the behavior of digital interlocutors
%questioning the ethical implications of machines and communicators

%A message exchanged between a co-present human and computer, for example, has been theorized as analogous to interpersonal (human) communication (e.g. Waddell et al., 2016).
%Within HMC, the question of “who is a person interacting with?” shifts to “what are they communicating with?” (Gunkel, 2012a).
%Therefore, ongoing research should not only be focused on assessing the similarities between humans and machines in their function as communicators, but should also take into account the differences, so that scholars can develop an understanding of technology as a unique type of communicator.

%Given that communicative AI has only recently become more available, much has yet to be learned regarding how people conceptualize and interact with these more advanced technologies within the context of their daily lives. Two key elements of communication theory are space and time (e.g. Innis, 2008), and future research could focus on how these elements factor into the function of AI as communicator and how people perceive it as such. For example, it is now possible to conduct longitudinal studies of how and the degree to which people’s conceptualizations of programs and devices as communicators change over time and across different contexts.


==> content/07newdiscussion2.tex <==
\section{Discussion}
\label{sec:Discussion}

Explainability is a new NFR that echoes the demand for more human oversight of systems \cite{Thiebes2020}. It can bring either positive or negative consequences across all quality dimensions: from users' needs to system aspects.
The impact of explainability on so many dimensions may be related to the fact that explainability can be viewed as an aspect of communication between systems and humans. Just like communication in human relationships can either strengthen relationships or harm them, depending on how it occurs in practice, we may apply the same principle to explainability. 

%Poor design choices towards explainability can negatively affect the relationship with the user (e.g., user experience issues), interfere on important quality aspects for a corporation (e.g., damaging the brand image and the customer loyalty), and bring disadvantages for the project or the system (e.g., increasing development costs or hindering system performance).

Despite the fact that the topic of explainability has increased in popularity as a result of the rapid development of autonomous and intelligent systems, the community still lacks guidance on how to create such systems. Building appropriate elicitation techniques and providing requirements engineers with adequate tools to capture explainability requirements are challenges that still need to be addressed. Our research results point to the importance of explainability in the NFR landscape, emphasizing the need for greater awareness of this topic as well as greater understanding of its meaning.

Research in RE can profit from insights of other disciplines when it comes to explainability. The fields of philosophy, psychology, and human-computer-interaction, for example, have long researched aspects such as explanations or human interaction with systems (see \cite{Miller2019} for an overview of research concerning explanations in several disciplines). At the same time, requirements engineers can contribute by studying how to include such aspects in systems and adapt development processes. This knowledge must be made available and integrated into the day-to-day development of systems.

We believe that our contributions can guide software professionals to understand the meaning, taxonomy, impact and characteristics of explainability, facilitating the conception and development of explainable systems. Our working definition for requirements engineers and software professionals brings up essential components of explainable systems that should be translated into requirements and the respective functionality. Defining these component factors facilitates the software engineering process, supporting the elicitation and specification of correspondent explainability requirements, as well as their verification and validation. Conceptual models are useful to abstract, comprehend and communicate information. Moreover, our catalogue can serve as checklist during elicitation and also during trade-off analysis, helping software engineers prevent conflicts between quality aspects and choose the best strategies for achieving the desired quality outcomes. Both artifacts contain information that may be used to turn explainability into a positive catalyst for other essential system qualities in modern systems.

%These artifacts can also help to recognize trade-offs and synergies between explainability and other quality aspects. As a result, software engineers may prevent conflicts between quality aspects and choose the best strategies for achieving the desired quality outcomes. 

Our literature review illustrates that there is still much to do in the field of NFRs. As systems are progressing towards ever-new application fields, we believe that there may be other emerging NFRs besides explainability. Among others, ethics, fairness, and legal compliance are all quality aspects that are gaining importance and should be better researched. More traditionally, we have identified that explainability can exhibit an impact on nearly all NFRs that can be found in the ISO 25010~\cite{ISO25010}: performance efficiency, usability, reliability, security, maintainability, and portability. As such, the importance of explainability needs to be further recognized. Our work is just a first step into this direction. A plausible next step would be to adjust existing catalogues to also incorporate explainability. Furthermore, our community needs to explore what kind of activities need to be incorporated to the software engineering process in order to accommodate the necessary steps towards building explainable systems. %With this work, we expect to have given a valuable input with regard to this new requirement.
 
%Indeed, aspects such as human-machine cooperation and mental model accuracy show that there are specific needs with regard to systems when they are used to support humans.

==> content/07newdiscussion2_copy.tex <==
\section{Discussion}
\label{sec:Discussion}

Explainability is a new NFR that echoes the demand for more human oversight of systems \cite{Thiebes2020}. It can bring either positive or negative consequences across all quality dimensions: from users' needs to corporate values to system aspects. Explainability's impact on so many important dimensions illustrates the growing need to keep explainability in mind while designing a system. To this end, our working definition for requirements engineers and software professionals brings up some aspects that should be explored and translated into requirements and the appropriate functionality to fulfill them. Defining the component factors of explainable systems facilitates the software engineering process, supporting the elicitation and specification of requirements, as well as the verification and validation of the corresponding explainability requirements.

If not properly designed, explainability can negatively affect the relationship with the user (e.g., user experience issues), interfere on important quality aspects for a corporation (e.g., damaging the brand image and the customer loyalty), and bring disadvantages for the project or the system (e.g., increasing development costs or hindering system performance). This kind of impact may be related to the fact that explainability can be viewed as an aspect of communication between systems and humans. Just like communication in human relationships can either strengthen relationships or harm them, depending on how it occurs in practice, we may apply the same principle to explainability.

When it comes to this, requirements engineers may benefit from the insights of other disciplines. The fields of philosophy, psychology, and human-computer-interaction, for example, have long researched aspects such as explanations or human interaction with systems (see \cite{Miller2019} for an overview of research concerning explanations in several disciplines). At the same time, requirements engineers can guide discussions about how to include such aspects in systems and how to adapt development processes. This knowledge, scattered across different areas, must be made available and integrated into the day-to-day development of systems. Artifacts such as the model and the catalogue proposed in this paper can synthesize this knowledge. These artifacts can also help to recognize trade-offs and synergies between explainability and other quality aspects. As a result, software engineers may prevent conflicts between quality aspects and choose the best strategies for achieving the desired quality outcomes. 

Our literature review illustrates that there is much to do in the field of NFRs. We did not only distill traditional NFRs from our review, but widened our focus to quality aspects in general. As systems are progressing towards ever-new application fields, we believe that there may be other emerging NFRs besides explainability. Indeed, aspects such as human-machine cooperation and mental model accuracy show that there are specific needs with regard to systems when they are used to support humans. Among others, ethics, fairness, and legal compliance are all quality aspects that are gaining importance and should be better researched. In this regard, other disciplines like philosophy, law, and psychology can, again, provide valuable insights for RE. 

More traditionally, we have identified that explainability can exhibit an impact on nearly all NFRs that can be found in the ISO 25010~\cite{ISO25010}: performance efficiency, usability, reliability, security, maintainability, and portability. As such, explainability occupies a prominent role in the NFR landscape. The importance of explainability needs to be further recognized. Our work is just a first step into this direction. An plausible next step would be to adjust existing catalogues to also incorporate explainability. With this work, we expect to have given a valuable input with regard to this new requirement.
 
%Despite the fact that the topic of explainability has increased in popularity as a result of the rapid development of autonomous intelligent systems, the community still lacks guidance on how to create such systems. Building appropriate elicitation techniques, providing requirements engineers with adequate tools to capture explainability requirements are challenges that need to be addressed to build explainable systems. Conceptual models are useful to abstract, comprehend and communicate information. Moreover, oOur catalogue can serve as checklist during elicitation and also during trade-off analysis. Both artifacts contain information that may be used to better visualize the impactThe information in our model information helps to understand the significance of explainability as a system quality and how to use it as a positive catalyst for other essential system qualities in modern systemsit can help achieve important qualities for future systems. Thus, we believe that the major contribution of our work is in providing artifacts and guiding the first steps toward building explainable systems. The major contribution of our work is to take a step towards facilitating the creation of explainable systems by providing artifacts that guide software professionals to first understand the meaning, taxonomy, impact and characteristics of these systems. 

